Sequential Discrete Action Selection via Blocking Conditions and Resolutions

In this work, we introduce a strategy that frames the sequential action selection problem for robots in terms of resolving \textit{blocking conditions}, i.e., situations that impede progress on an action en route to a goal. This strategy allows a robot to make one-at-a-time decisions that take in pertinent contextual information and swiftly adapt and react to current situations. We present a first instantiation of this strategy that combines a state-transition graph and a zero-shot Large Language Model (LLM). The state-transition graph tracks which previously attempted actions are currently blocked and which candidate actions may resolve existing blocking conditions. This information from the state-transition graph is used to automatically generate a prompt for the LLM, which then uses the given context and set of possible actions to select a single action to try next. This selection process is iterative, with each chosen and executed action further refining the state-transition graph, continuing until the agent either fulfills the goal or encounters a termination condition. We demonstrate the effectiveness of our approach by comparing it to various LLM and traditional task-planning methods in a testbed of simulation experiments. We discuss the implications of our work based on our results.

==> DEPRECATED_3-technical_overview.tex <==
\section{Technical Overview}
\label{sec:technical_overview}

\begin{figure*}[t!]
	\includegraphics[width=\textwidth]{figures/placeholder_page_width.png}
	\caption{}
	\label{}
	\vspace{-12pt}
\end{figure*}

Our task execution framework aims to shift from traditional task planning methodologies. Unlike classical approaches that rely on fully observable and static environment models, our framework is designed for dynamic, partially observable environments. It leverages a novel combination of behavior graphs, hierarchical predicate resolution functions, and interaction with large language models (LLMs) to navigate and adapt to the complexities of real-world scenarios.

\subsection{Core Components}
\subsubsection{Behavior Graphs and Hierarchical Predicate Resolution}

Central to our framework is a behavior graph structured as a series of hierarchical predicate resolution functions. This design enables the system to generate sets of feasible actions by resolving predicates that represent the current state of the environment as observed by the robot.
The hierarchical nature of the predicate resolution allows for an efficient search through possible actions, focusing on those most relevant to the robot's current context and objectives.

\subsubsection{Partially Observable State Representation}

The framework is specifically tailored to operate in partially observable environments. It does this by maintaining a dynamic representation of the environment through predicates known to be satisfied based on the robot's current perception.
This approach allows the robot to make informed decisions even with incomplete information, significantly enhancing its ability to adapt to unforeseen changes.

\subsubsection{Action Set Generation and LLM Query}

Upon determining feasible actions, the framework formulates a structured query to a Large Language Model (LLM). This query includes the sets of actions along with the current state representation.

The LLM then evaluates these options to select the most helpful action for the robot to take, given its current state and objectives. This process benefits from the LLM's vast knowledge base and its ability to make complex inferences.

\subsubsection{Failure Detection and Resolution}

An integral part of the framework is its robust failure detection mechanism. When unforeseen failures occur, the system can identify these incidents and insert temporary goals into the behavior graph to resolve the issue before returning to the primary objective.
This mechanism ensures that the robot can adaptively respond to challenges, maintaining progress toward its goals even in the face of unexpected obstacles.


\subsection{Advantages over Classical Task Planning}

Adaptability in Partially Observable Environments: By focusing on current, observable states, our framework is inherently more adaptable to dynamic environments than traditional methods that require a fully observable state.
Efficient Action Selection: The hierarchical structure of predicate resolution combined with LLM integration allows for an efficient and informed selection of actions, leveraging advanced AI to navigate complex decision spaces.
Robustness to Failures: The embedded failure detection and resolution capability provides a layer of resilience that classical planning methods often lack, enabling continuous operation under uncertainty.

